Characterizing and modeling the mechanical behavior of an anion exchange membrane for carbon capture applications

A new direct air capture (DAC) technology uses a moisture swing (MS) process with anion exchange membranes, potentially offering a more energy-efficient way to remove CO2 from the air. In this MS process, the membrane absorbs CO2 as it dries and releases it when water is added. Understanding the mechanical behavior of these membranes is essential for improving the design and efficiency of DAC systems and prolonging sorbent lifetime. This study tested one anion exchange membrane, Fumasep FAA-3, under mechanical loading and various temperature and humidity conditions to measure its swelling, stiffness, strength, plastic deformation, and stress relaxation. Experimental results were used to identify a mechanical model for FAA-3 that can be used to predict the material's nonlinear viscous behavior under various loads and environments.

==> 3_chapter2.tex <==
\chapter{Experimental Characterization}

\section{Introduction}
Ion exchange polymer membranes have various uses, such as fuel cells, batteries, and electrodialysis for water desalination \cite{SILBERSTEIN20105692}. A new potential application of ion exchange polymer membranes is the continuous separation of CO$_2$ from air for direct air capture, commonly termed DAC, a technology to remove the most abundant greenhouse gas (GHG) from the atmosphere. These materials have been shown to absorb/desorb CO$_2$ through a change in moisture \cite{MoistureSwingSorbent,kaneko2022kinetic,Wade}. 

The concept of DAC is not a new idea \cite{lackner1999carbon}, but the growing influence of climate change has made it a necessity. Carbon emissions stem from burning fossil fuels, food production, transportation, and deforestation. These factors have caused climate change to become an alarming problem. According to the World Health Organization (WHO), 37\% of heat-related deaths are due to climate change \cite{World_Health}. Compared to the average temperature of the late 19th century, the temperature of Earth has increased by approximately 2.45 degrees Fahrenheit (about 1.36 degrees Celsius) in 2023 \cite{NASA}. To combat the large inflow of CO$_2$, new renewable energy technologies are being employed to decarbonize the power and energy sectors. However, the slow rate of decarbonization and the need to treat the hard to abate CO$_2$ emissions to limit catastrophic warming necessitate the need for negative carbon emissions \cite{NAP25259}. DAC together with safe and permanent CO$_2$ sequestration is considered a potential approach to achieve net negative GHG emissions. However, most DAC technologies are still energy intensive and expensive \cite{DAC}. Moisture-swing polymer membranes are being considered for DAC to enable lower cost and more energy efficient separation \cite{castro2022new}.

Moisture-swing (MS) polymers contain anion exchange sites that can capture/release CO$_2$ by changes in water content \cite{MoistureSwingSorbent}. When dry, alkaline anions (carbonate or hydroxide) in these materials will chemically bind with CO$_2$ to form bicarbonate anions. When the bicarbonate anions are hydrated from either liquid water or water vapor, bicarbonate anions release CO$_2$, leaving behind a carbonate \cite{MoistureSwingSorbent}. Since the material is a membrane, the moisture swing process can be made efficient through continuous separation. By controlling moisture content throughout the material, one side of the membrane can be made dry for carbon capture and the other side can be made wet for carbon release and storage. In naturally dry environments, the dry side can be ambient conditions, and the DAC process can be continuous with minimal energy inputs.

Applications of polymer moisture-swing materials in the carbon capture process are currently limited by their slow absorption and desorption rate, low storage capacity, and the mechanical behavior of the polymer. Anion exchange materials are often brittle and may not last the desired lifespan for DAC. During the moisture-swing process, the material may be subject to repeated humidity and temperature cycling and in turn shrink/swell (or expand/contract) cycles, which can cause significant deformations and stresses that can lead to crack propagation and material failure. To better understand the mechanical behavior and prevent mechanical failure of the ion exchange MS materials, we aim to characterize and model the mechanical behavior of a commercially available moisture-swing, anion exchange membrane, Fumasep's FAA-3. FAA-3 is a lightly cross-linked polyphenylene oxide (PPO) polymer functionalized with quaternary ammonium charge sites charged balanced with bromide \cite{MOHANTY202027346}. The bromide is ion exchanged into an alkaline state (e.g. to CO$_3^{2-}$ or OH$^-$) to become reactive with CO$_2$. As a polymer, this material is expected to undergo permanent deformation and relaxation/creep, so modeling the mechanics of this material is not trivial. Specifically, this work examines the mechanical behavior of FAA-3, loaded with CO$_2$ in the bicarbonate state (FAA-3-HCO$_3$) through experimental tests and develops a model for the mechanical response of this material. 

The mechanical response of these membranes was investigated through similar anion exchanged materials to identify prior mechanical characterizations and gain insight into their behaviors. This analysis encompassed existing studies on FAA-3, poly(vinyl benzyl chloride)-based membranes (c(Je)-QAPVB), and other PPO-based anion exchange membranes \cite{Khalid,ZHENG2024854,narducci2016mechanical}. However, most characterizations of anion exchanged membranes are limited by simple stress-strain behaviors with swelling data that only entitles submerged conditions. Little data is provided on the strain rate and hydration/temperature effects of anion exchange membrane, and the viscous and plastic deformation responses that can occur within the material, exceptions include \cite{SILBERSTEIN20105692,YOON20113933,solasi2008time} but these are primarily for Nafion. Due to this, this study will examine the influence of these elements in detail within FAA-3 and use current existing anion exchange membrane results to verify similar properties and trends.

This study quantifies the tensile, cyclic, and time-dependent mechanical response of FAA-3-$\mathrm{HCO}_3^-$, including hydration and temperature effects. Additionally, we characterize the hydration swell and thermal expansion of FAA-3-$\mathrm{HCO}_3^-$ to identify the behavior in a continuous separation process where temperature and moisture are subject to dynamic changes. Using the mechanical behavior of FAA-3-HCO3 from these tests, we can identify a model that captures the rate, hydration, and temperature-dependent viscoplastic, stress-strain behavior during uniaxial tensile and cyclic loading conditions. An accurate mechanical model for anion exchange membranes can eventually be coupled with electrochemical transport to effectively predict and simulate the mechanical response of this moisture-swing material during the carbon capture process.  This in turn will predict the impact of chemical species transport on mechanical deformations during moisture swing cycles and vice versa.

\section{Materials and Methods}
This study examines the mechanical behavior of the MS responsive AEM using dynamic mechanical analysis (DMA) (sect \ref{sec:Dynamic Mechanical Analysis Test}), ultimate tensile (sect \ref{sec:Ultimate Tensile Test}), load-hold-unload (sect \ref{sec:Load-Hold-Unload Test}), and cyclic (sect \ref{sec:Cyclic Loading Test})loading experiments. All tests are conducted in tension and the loading direction is along the long edge of the membrane (in-plane) unless otherwise noted. DMA assesses the extent of the mechanical viscous effect, captures the storage and loss modulus, and identifies the glass transition temperature. The ultimate tensile tests characterize the strength, elastic modulus, and elongation at failure at various rates and humidities. The load-hold-unload tests characterize viscous effects during the hold and the amount of plastic deformation prevalent in the material during the unload. The cyclic tests mimic in-use conditions of hydration and temperature change as best as possible given experimental constraints and validate the accuracy of identified/developed models. In addition, tests without any mechanical load characterize the polymer's hygroscopic swell (sect \ref{sec:Hygroscopic Swell}) and thermal expansion (sect \ref{sec:Temperature Test}). The engineering strain of the material is decomposed into \begin{equation}
    \label{Eq Strain}
    \epsilon^{tot} = \epsilon^{mech} + \epsilon^{th} + \epsilon^{hygro},
\end{equation}
where $\epsilon^{tot}$ is the total engineering strain, $\epsilon^{mech}$ is the mechanical strain, $\epsilon^{th}$ is the thermal strain, and $\epsilon^{hygro}$ is the hygroscopic swelling strain. Eq. (\ref{Eq Strain}) demonstrates how the strain of the material is dependent on mechanical strain coming from applied forces, thermal strain from temperature changes, and hygroscopic strain from changes in water content, so it is important to individually characterize these behaviors to model the material. Most tests were performed on at least two samples to ensure repeatability. Details on the material and each of these tests are described subsequently.

\subsection{Materials}
\label{sec:Materials}
Commercially available Fumasep FAA-3 samples with a thickness of 30$\mu$m were used in this work. The sample membranes are received with a bromide counterion from the manufacturer. However, these samples will commonly be in a bicarbonate state to move active CO$_2$. To replicate the state in which the samples will be utilized, the FAA-3 samples are ion exchanged into a HCO$_3^-$ (bicarbonate) state. The original bromide-based sample is stirred in 0.1 M $\mathrm{kHCO}_3^-$
 solution for 24 h, rinsed with deionized (DI) water, and then soaked again in a stirred fresh solution of 0.1 M KHCO3 for 24 h to perform a bicarbonate ion exchange. The bicarbonate ion exchanged samples of FAA-3 specimens were equilibrated to ambient conditions, approximately \SI{23}{\celsius} and relative humidity (RH) of 30-40\%, before being cut into the dog-bone geometry shown in Figure \ref{fig:ASTM 1708}. The sample shape follows ASTM standards: ASTM D-1708 \cite{ASTM}. The dimensions have a gauge length of 12 mm and a width of 5 mm. Unless otherwise noted, this gauge length (12 mm) was used as the reference state for all strain calculations, and thus the reference state is under ambient conditions.

    \begin{figure}[hbt!]
        \centering
        \includegraphics[width=0.65\linewidth, height=0.3\textheight]{figures/ASTM 1708 dim.png}
        \caption{Schematic diagram of the ASTM D-1708, dog-bone sample geometry in millimeters adapted from \cite{ASTM}.}
        \label{fig:ASTM 1708}
    \end{figure}

\subsection{Dynamic Mechanical Analysis Test}
\label{sec:Dynamic Mechanical Analysis Test}
The dynamic mechanical analysis (DMA) test is an experiment designed to measure the mechanical properties of materials under oscillating stress or strain. By applying an oscillating force or displacement to the material and measuring the lag in response, the DMA can reveal the storage modulus (instantaneous elastic response), loss modulus (viscous response), and tan($\delta$) (damping factor) with the $\delta$ representing phase angle. Through the storage and loss modulus results, the dissipation characteristics as a function of temperature and the glass transition temperature can be determined. 
At the glass transition temperature, the storage modulus decreases dramatically, and usually, the loss modulus reaches its maximum. This temperature is important to know as the mechanical behavior changes significantly around this point and any model for the glassy behavior of the material is likely not applicable above this temperature. 

A TA Instruments Hybrid Discovery Rheometer 2 was utilized for the DMA testing of FAA-3. Figure \ref{fig:Rheometer} illustrates the rheometer setup for these tests. The rheometer can measure and control the force, displacement, and temperature of a sample within the machine. The force and displacement are controlled through the software by moving the upper clip attached to the sample. The temperature is controlled by blowing hot or cold fluids into the sample in a sealed chamber. The force resolution of the rheometer is 0.0005N, the temperature resolution is \SI{0.01}{\celsius}, and the displacement resolution is 0.02${\mu}$m. Although the sample was cut into dog-bone shapes for the experiments, in this test, the sample was rectangular with a length of 7.5 mm and a width of 12.5 mm. The dog-bone geometry was not used for this test since the purpose of this shape is to allow the applied force to be concentrated in the middle where the gauge length and width are located, but the sample expands with increasing temperature and this expansion also occurs outside of the gauge dimensions so a rectangular sample is used.

    \begin{figure}[hbt!]
        \centering
        \includegraphics[width=0.4\linewidth, height=0.38\textheight]{figures/Rheometer.png}
        \caption{Rheometer setup for DMA test.}
        \label{fig:Rheometer}
    \end{figure}
    
The DMA test performed on FAA-3 used a temperature sweep while the sample was cyclically loaded. The temperature sweep was from \SI{-150}{\celsius} to \SI{250}{\celsius} at a rate of \SI{3}{\celsius}/min. To get the low temperature of \SI{-150}{\celsius}, liquid nitrogen was used as the fluid blowing on the sample to cool it down. When the sample is inputted into the rheometer, before any loading, the chamber surrounding the sample is set to the lowest temperature of \SI{-150}{\celsius} and the sample is given \SI{20}{\minute} to equilibrate to its surrounding temperature and conditions. The cyclic load was at 1 Hz with an amplitude of 18${\mu}$m and an initial length of 7.76 mm. 

An additional conditioning step was implemented within the rheometer before the test. As the temperature increases, the material is expected to expand, and it is important to ensure that as the sample grows, it remains taut and does not buckle. Therefore, an initial force of 5 N was applied before any cyclic loading began and the force tracking function was used to keep the sample between a load of 5 N and a minimum load of 1 N to prevent the sample from buckling. Note that unlike all other tests, in the DMA, the length in the coldest state after applying the 5 N was considered the initial length, and this was 7.76 mm. This 5 N force proved to be enough so that even as the sample thermally expanded, the force never reached below 1 N, and the sample did not need additional tensile force applied during the temperature sweep.

\subsection{Hygroscopic Swelling}
\label{sec:Hygroscopic Swell}
The swell test was devised to determine the swell coefficient of FAA-3 during moisture absorption or desorption. Determining the swell coefficient ($\bm{\beta}$) is particularly important for MS DAC applications as moisture swing is the driving mechanism. This coefficient can be found through the hygroscopic strain, $\epsilon^{hygro}$, from Eq. (\ref{Eq Strain}). The $\epsilon^{hygro}$ can be related to changes in moisture content by \begin{equation}
    \label{Eq hygro}
    \epsilon^{hygro} = {\bm{\beta}\Delta}WC,
\end{equation}
where $\bm{\beta}$ is the swell coefficient from water and ${\Delta}WC$ is the change in water content \cite{Hygroscopic}. When FAA-3 absorbs water, ${\Delta}WC$ is positive, and $\epsilon^{hygro}$ is positive, indicating that the sample will begin to swell and enlarge. When the water evaporates and the sample dries up, ${\Delta}WC$ is negative, and according to Eq. (\ref{Eq hygro}), that implies $\epsilon^{hygro}$ is negative, so the sample will shrink. Therefore once $\epsilon^{hygro}$ is related to ${\Delta}WC$, $\bm{\beta}$ can be found.

To determine the swell coefficient, the material is not loaded mechanically (only a small mass was used to keep it taut) and measurements are made both in-plane and through the thickness. The swell response of the membrane in each direction is expected to be different due to the anisotropic nature of membranes \cite{Khalid}, so $\bm{\beta}$ will look like \begin{equation}
    \label{Eq beta}
    \bm{\beta} = 
    \begin{bmatrix}
        \beta_{in-plane} & 0 & 0 \\
        0 & \beta_{in-plane} & 0 \\
        0 & 0 & \beta_{thick}
    \end{bmatrix}
\end{equation}
where $\beta_{in-plane}$ is the swell coefficient in-plane which is expected to be different from $\beta_{thick}$, the swell coefficient through the thickness. The zeros in Eq. (\ref{Eq beta}) are because swell only causes normal strains, not shearing. Prior testing showed that the material was transversely isotropic so it was fair to assume that the swell coefficient would be the same in both in-plane directions.

Note that during MS DAC, it is expected that the thickness of the membrane will separate the wet and the dry condition, therefore $\beta_{thick}$ is of particular importance. Under these loading conditions, the membrane is expected primarily to be in bending due to expansion of the wet side and contraction of the dry side. Bending leads to axial stress, and therefore the mechanical behavior through the thickness is not particularly important, which is why only the swell tests take into account the anisotropy of the material and make measurements through thickness.

To measure swell in the in-plane and thickness directions, a humidity chamber was built. The sample is placed inside the chamber and is clipped at the top to keep it in place. A small mass (approximately 8.8g) was added to the bottom of the sample to keep it upright and taut. The humidity within the chamber is changed between ambient (32\% RH), 50\% RH, 80\% RH, and 90\% RH, and the sample in the chamber is given 24 h to equilibrate to this humidity. Once equilibrated, the length and thickness of the sample are measured to calculate the hygroscopic strain. An opening had to be made within the chamber when taking measurements, so the change in humidity when the chamber is opened for measurements is recorded as well. The length of the sample is measured with a caliper with an accuracy of $\pm$0.01 mm and measurements of the thickness were collected using a micrometer, with an accuracy of ${\pm}$0.001 mm. The dog-bone sample is not used since the portions of the sample outside the gauge dimensions are also swelling. Instead, a rectangular sample with a recorded length of 26.28 mm and thickness of 34$\mu$m in ambient conditions was used. The apparatus can be seen in Figure \ref{fig:Swell Test Setup}.

    \begin{figure}[hbt!]
        \centering
        \includegraphics[width=0.7\linewidth, height=0.3\textheight]{figures/Swell Test Setup.png}
        \caption{Swell test humidity chamber setup.}
        \label{fig:Swell Test Setup}
    \end{figure}
    
With the hygroscopic swell strain as a function of relative humidity, the change in water concentration needed to be related to relative humidity so that the change in water concentration could be related to strain and Eq. (\ref{Eq hygro}) could be employed. 

The water vapor sorption of the membrane was measured using a Discovery SA Dynamic Vapor Sorption Analyzer(TA Instruments, Delaware, USA) with a nitrogen purge rate of 20 mL/min. About 1-7 mg of the membrane films were used for each measurement. In this case, 50$\mu$m thick samples were used, but the samples were subject to the same bicarbonate exchange pretreatment. The samples were dried in the instrument at \SI{25}{\celsius} until the sample weight reached equilibrium ($<$0.01 wt\% change in 30 min, 4-12 h). Sample weight at equilibrium is recorded as the dry weight ($m_{dry}$). Relative humidity (RH) was then increased in 5\% steps from 0\% to 20\% RH, then 10\% steps from 20\% to 90\% RH. For each step, the sample was equilibrated for 8 h or until the change in sample weight was less than 0.01\% in 30 min. The water vapor uptake was measured with 3 distinct samples. The average uptake was reported with one standard deviation. The water vapor uptake fraction is calculated as \begin{equation}
    \label{Eq water uptake}
    uptake=\frac{(m-m_{dry})}{m_{dry}}
\end{equation}
%%
and the concentration (vapor uptake) over the relative humidity (water activity) data is seen in Figure \ref{fig:con vs hum}.

    \begin{figure}[hbt!]
        \centering
        \includegraphics[width=0.62\linewidth, height=0.35\textheight]{figures/concentration vs humidity.png}
        \caption{Water concentration of FAA-3 at equilibrated relative humidity \cite{Wade}.}
        \label{fig:con vs hum}
    \end{figure}

The water vapor sorption isotherm is fitted to the Park model \cite{park1986transport}: \begin{equation}
    \label{Eq water concentration}
    C=\frac{(A_L b_L a_w)}{(1+b_L a_w )}+k_H a_n+k_a a_w^n
\end{equation}
where C represents the total concentration of water, water activity is a$_n$, $A_L$, and $b_L$ are the Langmuir adsorption isotherm. $k_H$ is the Henry's Law constant, $k_a$ is the water aggregation reaction constant and $n$ is for water clustering. The model parameters and mean relative percentage deviation modulus ($D$) are shown in Table \ref{tab:Park model parameters}.


\begin{table} [hbt!]
    \centering
    \caption{Park model parameters for water concentration.}
    \label{tab:Park model parameters}
    \begin{adjustbox}{width=.7\textwidth}
    \begin{tabular}{|c|c|c|c|c|c|} \hline 
         $A_L$& $b_L$& $k_H$& $k_a$& $n$& $D$\\ 
         \hline 
         0.02264& 34.32& 0.1484& 0.2371& 6.241& 0.346\\ 
         \hline 
    \end{tabular}
    \end{adjustbox}
\end{table}


\subsection{Thermal Expansion}
\label{sec:Temperature Test}
Just as the material swells due to increased water content, temperature changes also lead to normal strains in the material. The thermal strain, $\epsilon^{th}$, can be related to changes in temperature by \begin{equation}
    \label{Eq temp}
    \epsilon^{th} = \alpha{\Delta}T,
\end{equation}
where $\alpha$ is a thermal expansion coefficient, and ${\Delta}T$ is a change in temperature from some reference temperature. Note that Eq. (\ref{Eq temp}) for thermal expansion is analogous to Eq. (\ref{Eq hygro}) for hygroscopic swell. However, in this case, the anisotropy of $\alpha$ will not be considered and only in-plane thermal swell will be measured. This is because thermal changes are expected to be minimal during the MS process.

The test was conducted in submerged conditions, with the axial strain being measured as the temperature of the water increased. The TA Instruments Hybrid Discovery Rheometer 2 (refer to section \ref{sec:Dynamic Mechanical Analysis Test}) was utilized to control/measure the force, position, and temperature. Although the temperature control of the rheometer was done with gases in the DMA test, the machine also can perform tests while having the sample submerged in a liquid. Submerging the samples in DI water ensures 100\% RH for all tests (heated air may have resulted in different humidities at different temperatures). To get a fast response of the fluid to changes in temperature, an external system was employed to heat the water. Figure \ref{fig:Rheometer Fluid} shows the hot plate used to heat the water needed for the test and the pump for circulating the fluid into and out of the container enclosing the sample. Before thermal loading, the sample was given \SI{15}{\minute} to equilibrate and swell in water. For the duration of the test, the force was set to near zero (a small force of 0.1-0.4N kept the specimen taut). The temperature began at ambient room temperature (\SI{21}{\celsius}) and was increased at a rate of approximately \SI{1}{\celsius}/min until it reached a value of \SI{40}{\celsius}

    \begin{figure}[hbt!]
        \centering
        \centering (a){{\includegraphics[width=0.3\linewidth, height=0.24\textheight]{figures/Rheometer Fluid 1.png}}}%
        \qquad
        \centering (b){{\includegraphics[width=0.4\linewidth, height=0.25\textheight]{figures/Rheometer Fluid 2.png}}}%
        \caption{Setup for submerged testing using an external hotplate to control temperature, (a) picture and (b) schematic.}%
        \label{fig:Rheometer Fluid}%
    \end{figure}
    
\subsection{Ultimate Tensile Test}
\label{sec:Ultimate Tensile Test}
The ultimate tensile test was conducted to obtain a general understanding of the polymer behavior and identify properties such as ultimate strength, elongation at failure, and elastic modulus. In addition, these tests were performed first to help identify load conditions for some of the other tests in this work. For example, the maximum strain in the load-hold-unload (section \ref{sec:Load-Hold-Unload Test}) was determined by results from the ultimate tensile tests to ensure that the material did not fail.

During these tests, an ELECTROPULS E3000 Instron was utilized to control the strain rate experienced by the sample. In this machine, a sample is clipped on both ends and pulled apart at a given force or displacement rate while recording both force and position. These results were used to calculate the stress and strain. The dog-bone shaped sample was attached to the top and bottom clips of the Instron, as shown in Figure \ref{fig:Instron Clips}.

    \begin{figure}[hbt!]
        \centering
        \centering (a){{\includegraphics[width=0.32\linewidth, height=0.27\textheight]{figures/Instron Clips.png}}}%
        \qquad
        \centering (b){{\includegraphics[width=0.42\linewidth, height=0.27\textheight]{figures/Instron Clips 2.png}}}%
        \caption{Experimental apparatus demonstrating the sample being held by upper and lower clips of the Instron (a) picture of test setup and (b) schematic.}%
        \label{fig:Instron Clips}%
    \end{figure}
    
The relative humidity and the temperature were tracked using a Govee Hygrometer Thermometer. The accuracy of the temperature is ${\pm}$\SI{0.3}{\celsius} and the accuracy of the humidity is ${\pm}$3\% RH.

Once set up, a nominal strain of approximately 0.2\% was applied to the sample to ensure was taut. %A to straighten the sample. 
The experimental procedure is then executed by pulling the sample in tension at the specified strain rate until the sample breaks.

\subsubsection*{Rate Variance}
\label{sec:Ultimate Tensile Test Rate}
The tensile tests were performed under constant engineering strain rates of 0.1s$^{-1}$ (fast) and 0.01s$^{-1}$ (slow), at room temperature and ambient relative humidity. Figure \ref{fig:Govee} shows the variations in temperature and humidity during tests. Note that they are relatively stable with minimal fluctuations due to environmental changes. Similar measurements were made for all other tests and showed similar fluctuations, and therefore are not presented.

    \begin{figure}[hbt!]
        \centering
        \centering (a){{\includegraphics[width=0.45\linewidth, height=0.25\textheight]{figures/Govee Temperature.png}}}%
        \qquad
        \centering (b){{\includegraphics[width=0.45\linewidth, height=0.25\textheight]{figures/Govee Humidity.png}}}%
        \caption{Govee hygrometer thermometer measuring (a) temperature and (b) humidity with natural fluctuations from the environment.}%
        \label{fig:Govee}%
    \end{figure}

\subsubsection*{Humidity Variance}
\label{sec:Ultimate Tensile Test Humidity}
The ultimate tensile test with varying humidity was performed under a constant engineering strain rate of 0.01s$^{-1}$ and at room temperature. To control the humidity, the Instron is equipped with a chamber that encloses the sample. Using salt solutions, as shown in Figure \ref{fig:Instron Setup}, the humidity within the chamber can be controlled. These solutions are mainly composed of deionized (DI) water and can be mixed with Potassium Nitrate to control the humidity of the chamber to a designated value. Some openings could not be fully sealed because the cross-head of the Instron needed to move freely to apply force/displacement to the sample. To account for these openings, the DI water and salt solutions were left in the chamber for 6 h until the chamber reached equilibrium. Once at equilibrium, the relative humidity was measured with a humidity sensor and recorded. The samples were then given 24 h to equilibrate in this condition before the tests were performed.

    \begin{figure}[hbt!]
        \centering
        \centering (a){{\includegraphics[width=0.3\linewidth, height=0.24\textheight]{figures/Instron Setup 1.png}}}%
        \qquad
        \centering (b){{\includegraphics[width=0.45\linewidth, height=0.25\textheight]{figures/Instron Setup 2.png}}}%
        \caption{Sealed Instron chamber with salt solutions to control humidity, (a) picture and (b) schematic.}%
        \label{fig:Instron Setup}%
    \end{figure}

To measure mechanical strain in these tests, assume that the material has length $L_i$ after equilibrating to the humidified environment, length $L_f$ at any instant during the test, and ${\Delta}L$ represents the change in length measured during the test relative to the humidified length (i.e. ${\Delta}L = L_f - L_i$). Temperature is not changing through these tests so the strain from temperature is zero. Referring back to Eq. (\ref{Eq Strain}), the mechanical strain, $\epsilon^{mech}$, is found as \begin{equation}
    \label{Eq mech}
    \epsilon^{mech} = \epsilon^{tot}-\epsilon^{hygro} = \frac{L_f-L_0}{L0}-\frac{L_i-L_0}{L_0}=\frac{L_f-L_i}{L_0}=\frac{{\Delta}L}{L_0}.
\end{equation}

\subsection{Load-Hold-Unload Test}
\label{sec:Load-Hold-Unload Test}
The load-hold-unload test was designed to observe the inelastic mechanical properties of FAA-3. Through this test, stress relaxation can be observed while the material is held with no change in position and plastic deformation is seen when the material is unloaded to a force near zero and residual strains remain. 

\subsubsection*{Humidity Variance}
\label{sec:Load-Hold-Unload Test Humidity}
For the load-hold-unload experiment, the sample is subject to the following: 1) loaded at the specified strain rate until the sample reaches a mechanical engineering strain of 1\%, 2) held in place for 1 minute, 3) unloaded to a force near zero at the same strain rate, 4) reloaded to a mechanical engineering strain of 5\%, 5) held in place for 1 minute, 6) unloaded to a force near zero, 7) reloaded to a mechanical engineering strain of 8\%, 8) held in place for 1 minute, and 9) unloaded to a force of zero. Note that the stress never fully went to zero during the test so the sample remained taut. Also, note that the mechanical strain was found by subtracting the strain due to hygroscopic swelling from the total strain, refer to Eq. (\ref{Eq mech}).

To observe how the material behavior changes with humidity, the test was conducted at ambient conditions (35\% RH - 40\% RH), approximately 70\% RH, and approximately 95\% RH. The test was done under a constant engineering strain rate of 0.01s$^{-1}$ and at room temperature of approximately \SIrange{23}{27}{\celsius}. The humidity-controlled samples were given 24 h in the humidity controlled environment to reach equilibrium.

These tests were performed using an Instron 8874 machine, which is similar to the ELECTROPULS E3000 Instron (refer to section \ref{sec:Ultimate Tensile Test Rate}). The major difference between the setup with the Instron 8874 as compared to the ELECTROPULS E3000 Instron is that the former has a load cell that has a 50N capacity for these tests while the latter has a 5kN load cell. This smaller load cell can more accurately measure and control the force applied to the sample and has an accuracy equal to or better than ${\pm}$ 0.25\% of the indicated force. This improvement is most apparent when unloading the sample; the large load cell unloads the sample to the original taut force with a deviation of around 1N, while the smaller load cell returns to the original taut force with a deviation of only around 0.1N. The position accuracy with system linear variable differential transformer (LVDT) (${\pm}$0.5\% of full scale) is ${\pm}$0.75 mm. The position resolution with system LVDT (1/500,000 of full scale) is 0.3 microns. The linear actuator stroke is ${\pm}$75mm. Strain is calculated from displacement using Eq. (\ref{Eq mech}). The Govee Hygrometer Thermometer continued to be used for temperature and humidity measurements, and as shown in Figure \ref{fig:Govee} small fluctuations were measured due to environmental changes.

    \begin{figure}[hbt!]
        \centering
        \centering (a){{\includegraphics[width=0.3\linewidth, height=0.21\textheight]{figures/Fluid Instron Setup 1.png}}}
        \qquad
        \centering (b){{\includegraphics[width=0.45\linewidth, height=0.21\textheight]{figures/Fluid Instron Setup 2.png}}}
        \caption{Instron fluid chamber for humidity control and submerge testing, (a) picture of test setup before the chamber is raised and (b) schematic.}%
        \label{fig:Fluid Instron Setup}%
    \end{figure}

\subsubsection*{Temperature Variance}
\label{sec:Load-Hold-Unload Test Temperature}
The load-hold-unload test with temperature variance was done under a constant engineering strain rate of 0.01 s$^{-1}$ and at 100\% RH (submerged). The loading procedure in this case was: 1) load to a mechanical engineering strain of 1\%, 2) hold in place for 1 minute, 3) unload to a force near zero, 4) reload to a mechanical engineering strain of 3.9\%, 5) held in place for 1 minute, 6) unload to a force near zero, 7) reload to a mechanical engineering strain of 9.8\%, 8) held in place for 1 minute, and 9) unload to a force of zero. 

Similar to Eq. (\ref{Eq mech}), the mechanical strain was found by subtracting the thermal strain from the total strain, \begin{equation}
    \label{Eq mech temp}
    \epsilon^{mech} = \epsilon^{tot}-\epsilon^{th}-\epsilon^{hygro} =\frac{{\Delta}L}{L_0}.
\end{equation}
where changes in length are relative to the thermally loaded and swelled state (i.e. ${\Delta}L = L_f - L_i$), and the initial length, $L_0$, is the gauge length before any thermal/hydro/mechanical loading. The temperature was changed between ambient (approximately \SI{19}{\celsius}), \SI{35}{\celsius}, and \SI{50}{\celsius}. These values were chosen because during MS DAC the material may be exposed to temperature changes due to the environment, so extreme heat/cold is not expected. The TA Instruments Hybrid Discovery Rheometer 2 (refer to section \ref{sec:Temperature Test}) was utilized for this experiment.

\subsection{Cyclic Loading Test}
\label{sec:Cyclic Loading Test}
The cyclic loading test was designated to simulate the hydration/dehydration condition of FAA-3 and to verify the model developed for the material. While experimental limitations prevent the change of moisture during a test, we can approximate moisture changes by subjecting the material to elongation/release cycles to mimic shrink/swell cycles that may be seen in MS DAC. Since the material takes time to absorb/desorb water during MS DAC, the cyclic loading test was performed at a strain rate of 0.0001 s$^{-1}$. This test was performed at room temperature and ambient relative humidity (approximately \SIrange{25}{28}{\celsius}
 and 37-41\% RH).

In these tests, the sample was loaded and unloaded for three cycles. The membrane is subject to the following: 1) loaded at the specified strain rate until an engineering strain of 8\%, 2) released until it reaches a force near 0, 3) reloaded back to an engineering strain of 8\%, 4) unloaded to a force near 0, 5) reloaded back to an engineering strain of 8\%, and 6) unloaded to a force of 0. These experiments were conducted using the Instron 8874 and the same experimental setup as in section \ref{sec:Load-Hold-Unload Test Humidity}.

\section{Results}
This section presents the results from the experimental tests used to characterize the mechanical behavior of FAA-3. The material’s response to applied loads, along with the influence of moisture and temperature on its behavior, are analyzed and documented. These results can help identify a model that accurately simulates the mechanics of FAA-3.

The results presented use engineering strain and nominal stress. Therefore, the term ``stress'' implies nominal stress, which is calculated using the reference area. For engineering strain, an additive decomposition is assumed using Eq. (\ref{Eq Strain}). The mechanical part of the engineering strain is often used to present results, as the model for the hygroscopic swell is given in Eq. (\ref{Eq hygro}) and the thermal expansion is given in Eq. (\ref{Eq temp}), thus only a model for the mechanical part must be determined. Moreover, the mechanical strain must capture the viscous effects and plastic deformation. The zero stress/strain state is after the material is taut, so while some stress may be present, it is neglected and all subsequent stress values are stresses above this minimal value to keep the specimen taut.

\subsection{Dynamic Mechanical Analysis Test}
\label{sec:Dynamic Mechanical Analysis Results}
The dynamic mechanical analysis (DMA) test performed reveals both the elastic and viscous material response of FAA-3 simultaneously through the storage modulus and loss modulus. 
%
    \begin{figure}[hbt!]
        \centering
        \includegraphics[width=0.7\linewidth, height=0.4\textheight]{figures/DMA results.png}
        \caption{Storage modulus, loss modulus, and damping factor over temperature from DMA testing }
        \label{fig:DMA results}
    \end{figure}
%
Figure \ref{fig:DMA results} shows that the storage modulus is greater than the loss modulus. However, the loss modulus values of 10$^8$ MPa are substantial, so viscous effects are prevalent within the material. Figure \ref{fig:DMA results} also shows that the storage and loss modulus are fairly steady throughout the range of temperatures tested, until near the end between \SIrange{200}{250}{\celsius}
. When the temperature reached \SI{200}{\celsius} and continued to increase to \SI{250}{\celsius}, the storage and loss modulus both showed a significant drop. The significant drop in storage modulus and the rise in damping factor (tan($\delta$)), the ratio of the loss modulus to the storage modulus, shows that a potential glass transition temperature may have been reached.

Even though the glass temperature could only be inferred to be around \SIrange{200}{250}{\celsius} by this test, the test confirmed that the glass transition temperature would not be in the operational range of temperatures. This is important for the applications because when FAA-3 is implemented for direct air capture, the material may be subjected to the temperatures of the surrounding environment (approximately \SIrange{0}{50}{\celsius}). If the glass temperature is within this ambient temperature range, it would make studying the mechanical behavior more difficult as going through the glass transition temperature would have a significant impact on the material properties.

One factor that made the DMA test conducted differ from regular DMA tests is the initial load applied to the sample. Typically, DMA tests only apply a sinusoidal strain. A force of 5N was applied in this case because of the thermal expansion the material undergoes when it is exposed to heat (seen in section \ref{sec:Temperature Results}) and the need to keep the specimen taut. As the temperature increased, the force on the specimen decreased due to the elongation of the specimen and the prescribed strain loading. In addition, the storage modulus results were significantly higher than expected for a polymer and higher than the Young's modulus seen in subsequent tests (e.g., see section \ref{sec:Ultimate Tensile Results}). However, the values obtained are not entirely unreasonable since there are anion exchanged membranes that have modulus in the GPa range, such as an anion exchange polymer based on Polysulfone (PSU) quaternized with trimethylamine (TMA) that has a modulus of 1440 MPa \cite{narducci2016mechanical}. Moreover, the difference in modulus between the high value obtained from DMA and the other results may be due to the rate of loading.

\subsection{Hygroscopic Swell}
\label{sec:Hygroscopic Swell Results}
The strain of the sample at various humidities was determined in the in-plane and thickness direction at room temperature of \SIrange{18}{20}{\celsius}. The measured relative humidity was correlated with the water content using the data in Figure \ref{fig:con vs hum}. The resulting hygroscopic swell strain as a function of changes in water concentration levels is seen in Figures \ref{fig:Swell Test Results In Plane} and \ref{fig:Swell Test Results Thickness}.

    \begin{figure}[hbt!]
        \centering
        \includegraphics[width=0.78\linewidth, height=0.43\textheight]{figures/Swell Test results in plane.png}
        \caption{Hygroscopic swell strain in the in-plane direction over the change in water concentration.}
        \label{fig:Swell Test Results In Plane}
    \end{figure}

    \begin{figure}[hbt!]
        \centering
        \includegraphics[width=0.76\linewidth, height=0.43\textheight]{figures/Swell test results in thickness.png}
        \caption{Hygroscopic swell strain in the thickness direction over the change in water concentration.}
        \label{fig:Swell Test Results Thickness}
    \end{figure}

As seen in Figures \ref{fig:Swell Test Results In Plane} and \ref{fig:Swell Test Results Thickness}, ranges were measured for both change in water concentration and strain. When measuring the dimensions of the sample, an opening in the humidity controlled chamber was made to accommodate the measurement tools, leading to a small drop in humidity within the chamber. In addition, the sample was difficult to measure as it was hanging upright, so 4-6 measurements were recorded in each direction. Therefore, the data points shown in Figures \ref{fig:Swell Test Results In Plane} and \ref{fig:Swell Test Results Thickness} represent the average measurement and the the solid black lines show the range of values measured for both strain and change in water content.

The relationship between change in concentration and swell strain is approximately linear, and the swell coefficient ($\bm{\beta}$) was determined to be 1.02x10$^{-5}$ m$^3$/mol in the in-plane direction and 9.24x10$^{-6}$ m$^3$/mol in the thickness direction. The swell coefficient ($\bm{\beta}$) quantifies the relationship between change in water concentration and swell strain. By determining this value, the swell strain in the in-plane direction and thickness direction can be found when there is a change in water concentration within FAA-3. Khalid et al. also measured the swell behavior of FAA-3 but they only captured two points (dry and wet) so a linear trend was employed to fit the data \cite{Khalid}. The swell test conducted in this study confirmed this relationship. However, one big difference between the result of Khalid et al. and the hygroscopic swell test results was that much more anisotropy was seen by Khalid et al. The swelling in the in-plane direction was approximately 15\% and 43\% in the thickness direction at a temperature of \SI{30}{\celsius}. The results from the hygroscopic swell experiment in this report were around 11\% in both directions at a constant change in concentration of 11026 mol/m$^3$ and a temperature of \SI{18}{\celsius}. Potential reasons for this difference could be the accuracy of the measurement tools implemented since the results from the thickness direction were measured by hand with a micrometer, which could be less accurate than the thickness gauge equipped with disc-shaped sensors used by Khalid et al. Furthermore, Khalid et al.'s sample (50$\mu$m) was thicker than the 30$\mu$m used for measurements in this paper so the thicker sample may have been easier to measure. In addition, the temperature in this study was approximately \SI{19}{\celsius} versus the \SIrange{23}{27}{\celsius} of the Khalid study. With the elevated temperature of Khalid's work, additional swelling seems likely. As molecules vibrate more at higher temperatures, there is more room for water molecules to penetrate and swell the material. This may explain the difference in the in-plane swell between this work and the work of Khalid et al. For the difference in the thickness swell, FAA-3 may be more anisotropic at higher temperatures. However, it seems more likely that the material was softer with the increase in temperature, and thus, the thickness is more likely to be underestimated (and thus, strain is overestimated) due to the squeezing of the material while measuring. Future work may consider optical measurements of thickness swelling strain to avoid this potential measurement error.

\subsection{Thermal Expansion}
\label{sec:Temperature Results}
The thermal expansion of FAA-3 was analyzed from ambient room temperature of \SI{21}{\celsius} to \SI{40}{\celsius} submerged in DI water. These tests should be performed under zero force (free expansion) but we applied a small 0.4N force to keep the sample taut. The relationship between change in temperature and strain is shown in Figure \ref{fig:Thermal Expansion Results}, with the reference temperature being the ambient conditions of \SI{21}{\celsius}.

    \begin{figure}[hbt!]
        \centering
        \includegraphics[width=0.8\linewidth, height=0.43\textheight]{figures/Thermal Expansion.png}
        \caption{Thermal expansion versus change in temperature with a linear fit.}
        \label{fig:Thermal Expansion Results}
    \end{figure}

When the temperature is increased, the molecules will vibrate more and move farther apart, thus the thermal strain. This trend is consistent with the DMA results since the sample also expanded with the increasing temperature in the DMA test until it eventually buckled, which is why a 5N force was applied to the sample for the test. The thermal expansion coefficient ($\alpha$) is determined through a linear fit of the experimental data (Figure \ref{fig:Thermal Expansion Results}). This was determined to be approximately 5.07x10$^{-3}$/\SI{}{\celsius}. %With this value, the strain caused by temperature can be calculated for the sample. T
he standard error of fit (S$_{yx}$) for the two curves was around 0.0055. A higher order model can be used to more accurately relate strain and temperature.
%
    \begin{figure}[hbt!]
        \centering
        \includegraphics[width=0.8\linewidth, height=0.41\textheight]{figures/Thermal Expansion 2.png}
        \caption{Thermal expansion versus change in temperature with a quadratic fit.}
        \label{fig:Thermal Expansion Results 2}
    \end{figure}
%
Figure \ref{fig:Thermal Expansion Results 2} shows a quadratic fit between temperature and engineering strain. The quadratic fit had a standard error of fit (S$_{yx}$) of 0.0026 for both curves. It can be seen through the lower S$_{yx}$ value that the quadratic fit for the trend of thermal expansion was much better than the linear trend. The quadratic relationship between thermal strain and change in temperature is 
\begin{equation}
    \label{Eq temp quad}
    \epsilon^{th} = \alpha_1{\Delta}T^2 + \alpha_2{\Delta}T,
\end{equation}
where $\alpha_1$ and $\alpha_2$ are the thermal expansion coefficient. From Figure \ref{fig:Thermal Expansion Results 2}, $\alpha_1$ is approximately 1.31x10$^{-4}$/\SI{}{\celsius}$^2$ and $\alpha_2$ is approximately 3.26x10$^{-3}$/\SI{}{\celsius}. 

In Khalid et al.'s results, the material size increased with temperature and this relationship was non-linear \cite{Khalid}. Although the trend was not quantified, it appears to be a quadratic, similar to what is seen in Figure \ref{fig:Thermal Expansion Results 2}.

\subsection{Ultimate Tensile Test}
\label{sec:Ultimate Tensile Results}
\subsubsection*{Rate Variance}
\label{sec:Ultimate Tensile Rate Results}
The uniaxial tensile behavior of FAA-3 during loading at ambient conditions (approximately \SI{23}{\celsius}, 41-43\% RH) contains a linear region at strains less than approximately 6\%, followed by a nonlinear region which includes the maximum stress experienced by material and fracture, as shown in Figure \ref{fig:Rate Ultimate Tensile Test eng}. 

    \begin{figure}[hbt!]
        \centering
        \includegraphics[width=0.80\linewidth, height=0.42\textheight]{figures/Rate Ultimate Tensile Test eng.png}
        \caption{Ultimate tensile test nominal stress versus the mechanical part of the engineering strain at engineering strain rates of 0.1s$^{-1}$ (fast) and 0.01s$^{-1}$ (slow), at \SI{23}{\celsius} and 42\% RH.}
        \label{fig:Rate Ultimate Tensile Test eng}
    \end{figure}

The strain rate in which the sample is loaded influences the maximum elongation and maximum stress with faster strains leading to more stress and elongation. This is expected since viscous effects lead to stress relaxation with time. Despite the change in strain rate, the initial, linear region, and the general shape of the graphs were similar. Table \ref{tab:Ultimate Tensile Test} provides the values of key parameters such as maximum stress, the slope of the linear region (Young’s modulus), and elongation at break under various conditions. 

\begin{table} [hbt!]
    \centering
    \caption{Mechanical properties of FAA-3 found using stress and engineering strain from the ultimate tensile test.}
    \label{tab:Ultimate Tensile Test}
    \begin{adjustbox}{width=\textwidth}
    \begin{tabular}{|c|c|c|c|c|c|c|c|} \hline 
         & Fast 1& Fast 2& Slow 1& Slow 2 & Humidified 1& Humidified 2& Humidified 3\\ 
         \hline 
         Rate (s$^{-1}$):& 0.1& 0.1& 0.01& 0.01& 0.01& 0.01& 0.01\\ 
         \hline 
         Humidity (\%):& 43.2& 42.2& 41.2& 41.4& 67.9& 71.8& 73.5\\ 
         \hline 
         Temperature (\SI{}{\celsius}):& 22.9& 23.2& 23.4& 23.5& 22.2& 22.1& 22.0\\ 
         \hline 
         Maximum stress (MPa):& 53.76& 52.66& 50.52& 48.83& 41.31& 34.49& 32.30\\ 
         \hline 
         Young’s Modulus (MPa):& 693.76& 692.88& 696.06& 703.81& 486.01& 403.77& 383.31\\ 
         \hline 
         Mechanical strain at break (\%):& 14.88& 12.77& 13.11& 13.00& 20.95& 12.90& 13.45\\ 
         \hline
         Swell (\%):& N/A& N/A& N/A& N/A& 7.03& 6.7& 8.22 \\ 
         \hline
    \end{tabular}
    \end{adjustbox}
\end{table}

The Young’s Modulus determined from the results was close to 700 MPa, demonstrating that the strain rate did not influence the linear-elastic region of the membrane. The ultimate tensile strength was around 53 MPa for the faster strain rate of 0.1s$^{-1}$ and around 50 MPa for the slower strain rate of 0.01s$^{-1}$. The average strain the sample reached before fracturing was 13.82\% at the faster rate and 13.06\% at the slower rate. These results show that in the range of rates tested, the strain rate had little influence on the overall tensile properties of FAA-3 since the values were relatively similar for all the properties. 

Comparing the resulting modulus to the storage modulus from the DMA (refer to section \ref{sec:Dynamic Mechanical Analysis Results}) the values were smaller. The Young's modulus from the ultimate tensile test was around 700 MPa at an ambient temperature of \SI{23}{\celsius}, while the storage modulus from the DMA test was around 1.5 GPa at approximately \SI{23}{\celsius}. Potential reasons for the variance could be from the 5N force applied that would normally not occur for DMA testing and the faster rate of the oscillating load. The fast rate from the DMA could have caused a greater storage modulus since the rapid oscillating load would not allow for as much relaxation to occur so the material appears stiffer. 

\subsubsection*{Humidity Variance}
\label{sec:Ultimate Tensile Humidity Results}
Although the mechanical behavior of FAA-3 did not vary much with strain rate, the change in relative humidity has a noticeable impact, seen in Figure \ref{fig:Humidity Ultimate Tensile Test eng}.

    \begin{figure}[hbt!]
        \centering
        \includegraphics[width=0.8\linewidth, height=0.42\textheight]{figures/Humidity Ultimate Tensile Test eng.png}
        \caption{Ultimate tensile test nominal stress versus mechanical part of the engineering strain at various humidities and a temperature of \SIrange{22}{23}{\celsius}.}
        \label{fig:Humidity Ultimate Tensile Test eng}
    \end{figure}

Although both the ambient and high humidity samples still contain a linear region and a non-linear region, the maximum stress is decreased and the elastic region has a smaller slope when humidity is increased. This is expected as humidity degrades mechanical properties in other materials, such as wood \cite{wood} and other polymers like poly(methyl methacrylate) (PMMA) \cite{PMMA}. When water is absorbed into the material, it lubricates the polymer chains and disrupts the bonds between the molecules, and this can cause the stiffness and strength of the material to decrease \cite{betts2013anatomy,clark2018biology}. Table \ref{tab:Ultimate Tensile Test} provides the values of each key parameter obtained from Figure \ref{fig:Humidity Ultimate Tensile Test eng}. 

High humidity results caused a decrease in the maximum stress and Young’s Modulus, while the mechanical strain at break was generally similar for all humidities. This consistent engineering strain at break suggests that the failure of the material might stem from breaking the cross-link bonds. The cross-link bonds act as fixed points within the polymer chain and are the most likely sites to fail when the material is stretched to its limit, irrespective of the surrounding moisture conditions. The cross-linking is a covalent bond and covalent bonds are generally unaffected by water, so this could be the cause of the similar point of failure. Note that the first high humidity test did show significantly more elongation at break, but additional testing was unable to confirm this, signifying the first test may have been an outlier.

Also note that the elongation at break in Table \ref{tab:Ultimate Tensile Test} is the mechanical engineering strain at break. The overall strain the sample experiences at high RH is much greater than ambient conditions since the sample elongated by as much as approximately 7\% before any mechanical load was applied because of the hygroscopic swell. 

The trends in the results correlate with the FAA-3 testing by Khalid et al. \cite{Khalid}. Khalid et al. found decreasing tensile strength, decreasing Young's modulus, and increasing elongation at break with increasing humidity and temperature \cite{Khalid}. Along with this behavior, Khalid et al. found that the sample will become more ductile, making it more likely to stretch a longer length before
breaking as temperature and humidity increase. Although the trends among the results are generally consistent, the values obtained for each of the properties differ significantly. Table \ref{tab:Property comparison} compares the results from this work with Khalid et at. and other studies on anion exchanged membranes.

\renewcommand{\arraystretch}{5}
\begin{table} [hbt!]
    \fontsize{100pt}{9pt}\selectfont
    \centering
    \caption{Mechanical properties of anion exchange materials.}
    \label{tab:Property comparison}
    \begin{adjustbox}{width=\textwidth}
    \begin{tabular}{|c|c|c|c|c|c|c|c|} \hline 
         Author& Material& Rate (s$^{-1}$):& Humidity (\%RH):& Temperature (\SI{}{\celsius}):& Maximum stress (MPa):& Young’s Modulus (MPa):& Max Mechanical Strain (\%)\\
         \hline
         This Work& FAA-3-30-HCO$_3$& 0.01 & 42& 23& 53& 700&13\\
         \hline
         This Work& FAA-3-30-HCO$_3$& 0.01 & 72& 23& 33& 400&13\\ 
         \hline 
         Khalid et at. \cite{Khalid}& FAA-3-50-Cl& 0.004& 50-70& 23-27& 16& 520& 40\\ 
         \hline 
         Khalid et at. \cite{Khalid}& FAA-3-50-Cl& 0.004& 100& 30& 14& 75& 100\\ 
         \hline 
         Kushner et al. \cite{kushner2016side}& QA-PPO: BTMA40& -& 40& 24& -& 1000& -\\ 
         \hline 
         Kushner et al. \cite{kushner2016side}& QA-PPO: BTMA40& -& 70& 24& -& 700& -\\ 
         \hline
         Zheng et al. \cite{ZHENG2024854}& c(Je)-QAPVB-6.25 AEM& -& 70& 25& 13& -& 15\\
         \hline
         Zheng et al. \cite{ZHENG2024854}& c(Je)-QAPVB-12.5 AEM& -& 70& 25& 6& -& 18\\
         \hline
         Narducci et al. \cite{narducci2016mechanical}& PSU-TMA-HCO$_3$& -& 50& 25& 44& 985&10\\
         \hline
         Narducci et al. \cite{narducci2016mechanical}& PSU-TMA-OH& -& 50& 25& 20& 680&11\\
         \hline
    \end{tabular}
    \end{adjustbox}
\end{table}
While the values between each anion exchange material differ from one another, Table \ref{tab:Property comparison} shows that anion exchange membranes generally have a Young's modulus between 500-1000 MPa at \SI{25}{\celsius} and 40\% RH. For FAA-3, The tensile strength in dry conditions (50-70\% RH and \SIrange{23}{27}{\celsius}
) from Khalid et at. was much smaller than the experimental results in this work at 72\% RH and \SI{23}{\celsius}, while the elongation at break at dry from Khalid et at. was much greater than the experimental results in this work. The Young's modulus at 70\% RH were similar. The other values in Khalid et at. could not be used for comparison as their experiments were done while changing both the water content and temperature simultaneously. The load rate applied by Khalid et al. was at a rate of 0.004 s$^{-1}$ (0.17 mm s$^{-1}$), which is slower than the 0.01 s$^{-1}$ (0.12 mm s$^{-1}$) applied in our experiment, but likely not enough to explain the difference is strength and elongation. Note that the strain rate was not specified by Khalid et al., thus the strain rate of 0.004 s$^{-1}$ in Table \ref{tab:Property comparison} was calculated using the dimensions reported by Khalid et al. (4 x 1 cm$^2$) and assuming that 4 cm was the length in the direction of load.

Potential factors that could lead to these discrepancies between this work and Khalid et al.'s work is the difference in sample preparation and load. The samples utilized in this paper are bicarbonate exchanged FAA-3 samples, while Khalid et al. use a chloride exchanged FAA-3 samples. This difference in the ion exchange can be the cause of the significant variation in properties because Khalid et al. had compared their chloride exchanged results with prior results from hydroxide exchanged membrane and they saw significantly more swelling in the chloride exchanged FAA-3 samples \cite{Khalid}. For dry samples in the experiments, Khalid et al. first used a vacuum at \SI{60}{\celsius} to dry their samples for 24 h before letting the samples equilibrate to lab atmosphere (temperature of \SIrange{23}{27}{\celsius} and humidity of 50-70\%) for 2-3 hours. In this work, significantly more time is allocated for samples to equilibrate to the environment and the ambient humidity was much lower. Moreover, while a vacuum allows the sample to be dried much more than at room conditions, it can cause a change in the behavior of FAA-3 by breaking its polymer chains through a hydroxide degradation mechanism \cite{hickner2013anion}. 

The discrepancies in material properties became even more pronounced when compared to the other materials listed in Table \ref{tab:Property comparison}, as those experiments do not utilize FAA-3. Nonetheless, these results show that the Young's modulus, strength, and elongation at break are similar for FAA-3 compared to other anion exchange materials. FAA-3 does have a higher strength than other anion exchange membranes, but that may be because the tests were performed in Arizona, USA, where the ambient humidity is much lower than most temperate climates, and indeed those who reported lower strength all did so at higher humidities. It was also shown by Narducci et al. \cite{narducci2016mechanical} that bicarbonate exchanged materials have higher strength and stiffness values compared to other forms of anion exchanged materials, which could support the high values seen in bicarbonate exchanged FAA-3. The maximum mechanical strain of FAA-3 differed from Khalid et al. but was in line with others. While differences in elongation for the submerged tests can be explained by the water disrupting the bonds and lubricating slip between the chains, Khalid et al. also saw significantly more elongation than others for dry materials.

\subsection{Load-Hold-Unload Test}
\label{sec:Load-Hold-Unload Results}
\subsubsection*{Humidity Variance}
\label{sec:Load-Hold-Unload Humidity Results}
The results from the load-hold-unload test in Figure \ref{fig:Humidity LHU 1 eng} show the effects the relative humidity has on mechanical behavior, including viscous effects (hold) and plastic deformation (unload). 

    \begin{figure}[hbt!]
        \centering
        \includegraphics[width=0.8\linewidth, height=0.42\textheight]{figures/LHU 1 eng.png}
        \caption{Load-hold-unload test nominal stress versus the mechanical part of the engineering strain, at various humidities and temperature range of \SIrange{23}{27}{\celsius}.}
        \label{fig:Humidity LHU 1 eng}
    \end{figure}

The experimental results were at an ambient temperature (ranging from \SIrange{23}{27}{\celsius}) and at a low, medium, and high relative humidity. However, due to a lack of precise control of humidity, there is a range for each category: low or ambient RH is 35-40\% RH, medium RH is 75-85\% RH, and high RH is 90-95\% RH. The load of the load-hold-unload test reveals the same trend as the ultimate tensile test. As seen in Figure \ref{fig:Humidity LHU 2 eng}, the force required to pull the material to a certain strain decreases the higher the relative humidity. At ambient relative humidity of 36.7\% RH and 37.5\% RH, the sample reached a stress of approximately 56-58 MPa at a mechanical engineering strain of 8\%. This value decreased with an increase in humidity and when the sample was around 93-95\% RH (high), the stress of the sample at 8\% mechanical engineering strain was approximately 13-15 MPa. The Young’s Modulus also decreased with humidity: the Young’s Modulus is around 1007-1011 MPa in ambient RH and high humidity (90\%-95\%) is around 244-332 MPa. These values are all within range of others (see Table \ref{tab:Property comparison}), and trends seen previously (section \ref{sec:Ultimate Tensile Results}). Although the ambient modulus increased compared to the ultimate tensile test, this may be due to the lower ambient humidity of 37\%RH in these load-hold-unload compared to the ambient humidity of 42\%RH in the ultimate tensile test. This emphasizes the importance of humidity on the material since small changes in humidity can cause variations in the mechanical properties.

    \begin{figure}[hbt!]
        \centering
        \includegraphics[width=0.8\linewidth, height=0.4\textheight]{figures/LHU 2 eng.png}
        \caption{Load-hold-unload test the mechanical part of the engineering strain and stress over time, at various humidities and temperature range of \SIrange{23}{27}{\celsius}.}
        \label{fig:Humidity LHU 2 eng}
    \end{figure}

The hold component examines the stress relaxation that occurs when held at a constant strain. The relaxation that happens when held in place for a minute decreases with the increased humidity and is most notable at higher strains. This may be because the stress is less at higher humidities so there is less relaxation. Furthermore, the rate of stress relaxation does not appear to be dramatically different at various humidities. Looking at Figure \ref{fig:Humidity LHU 2 eng}, it can be seen how at 1\% mechanical engineering strain, the stress that decreased while being held changed by a very small amount. On the other hand, the amount of stress that decreased when held at higher strains was much greater at ambient humidity than a high humidity. This is a reasonable expectation since an engineering strain of 1\% is close to its original length, causing there to be little relaxation to occur. While at higher strains, the sample has significantly stretched past its original length so viscous effects are more prevalent and the stress relaxation is much more significant.

The unload assesses any permanent (plastic) deformation. When the loaded sample was released to a force close to zero (but non-zero to keep the sample taut), it was found that the plastic deformation of FAA-3 increased with increasing humidity. The sample had little deformation in ambient conditions and was almost able to return to its original length after being strained to 1\%. With an increase in mechanical strain to 5\% and 8\%, the amount of permanent deformation increased, and the sample did not return to its original length. These trends remained as the humidity was increased, but the plastic deformation was much greater. As seen in Figure \ref{fig:Humidity LHU 1 eng}, the residual strain in the sample when the force returned to a very small value was larger at higher relative humidity values. Again, this may be due to water lubricating the chains and disrupting some bonds, making slipping between chains easier.

These results are significant since FAA-3 will be loaded axially in DAC for continuous separation by clipping the edges of the membrane and making one side of the membrane wet and the other dry. This will result in bending as one side swells from water while the dry side does not. At the site where the FAA-3 is held in place, the material will want to swell but cannot. This will result in significant stresses at these locations, but the stresses should relax with time. Then, when/if the DAC process is stopped or paused, there will be permanent deformation of the material. These results show how much plastic deformation may occur depending on the water concentration.

\subsubsection*{Temperature Variance}
\label{sec:Load-Hold-Unload Temperature Results}
The influence of temperature was examined through the load-hold-unload tests of FAA-3 submerged in DI water. By submerging the sample, it can ensure that the relative humidity can be kept at a constant value of 100\% RH. The temperature effects on FAA-3 are shown in Figure \ref{fig:Temp LHU 1 eng}. Note that this data had a relatively slow sampling rate leading to the waviness in the results.

    \begin{figure}[hbt!]
        \centering
        \includegraphics[width=0.8\linewidth, height=0.42\textheight]{figures/LHU submerge 1 eng.png}
        \caption{Load-hold-unload test results for nominal stress versus the mechanical part of the engineering strain at various temperatures in submerged DI water.}
        \label{fig:Temp LHU 1 eng}
    \end{figure}

Like the load-hold-unload test results in the humidity variance (section \ref{sec:Load-Hold-Unload Humidity Results}), the load reveals the Young's modulus, the hold shows stress relaxation, and the unload shows plastic deformation. The trends shown with increasing humidity were also prevalent with increasing temperature. As seen in Figure \ref{fig:Temp LHU 2 eng}, the load required to pull the material to a certain strain decreases when the temperature is increased. When the sample was in the ambient water temperature (\SI{19}{\celsius}), the sample was able to reach a maximum stress of approximately 9 MPa at an engineering strain of 9.8\%. When the temperature was increased to \SI{35}{\celsius}, the maximum engineering stress of the material was 5.9 MPa at an engineering strain of 9.8\%. This trend remained as the temperature increased to \SI{50}{\celsius}, demonstrating that the modulus decreases when the temperature is increased. Thus, the material becomes less stiff with rising temperature and becomes more ductile as the temperature is increased. This is consistent with the DMA results since the storage modulus decreased with the rising temperature, signifying how the stiffness of the material decreases with increasing temperature.

    \begin{figure}[hbt!]
        \centering
        \includegraphics[width=0.8\linewidth, height=0.4\textheight]{figures/LHU submerge 2 eng.png}
        \caption{Load-hold-unload test the mechanical part of engineering strain and stress over time at various temperatures in submerged DI water.}
        \label{fig:Temp LHU 2 eng}
    \end{figure}

The hold components showed that stress relaxation decreased with temperature. The trend of the relaxation remained the same among the temperatures with the initial stress relaxation being the greatest and gradually leveling out with time. The amount of stress relaxation also increased with strain, which is expected since there is more stress to relax. For the third cycle at an ambient temperature (\SI{19}{\celsius}), the stress relaxation was approximately 4.7 MPa. For the same third cycle at \SI{50}{\celsius}, the stress relaxation was approximately 1.1 MPa. The change in stress relaxation was relatively small but a decrease was observed when the temperature was increased. However, when comparing the change in stress relaxation between varying temperatures and varying humidity, it can be seen that the change in humidity has a much greater impact. Looking at the results in section \ref{sec:Load-Hold-Unload Humidity Results}, the stress relaxation at ambient RH (37\% RH) was approximately 22MPa, and stress relaxation at 95\% RH was approximately 5 MPa. This shows that for the conditions in which FAA-3 will be applied, humidity has a much larger influence on stress relaxation than temperature. This implies that material parameters associated with stress relaxation and viscous effects may not need to be temperature-dependent. These trends can be further examined in Figures \ref{fig:Hum sub LHU 1} and \ref{fig:Hum sub LHU 2}, which shows the first cycle of the load-hold-unload test with humidity varying from ambient to submerged.

    \begin{figure}[hbt!]
        \centering
        \includegraphics[width=0.8\linewidth, height=0.42\textheight]{figures/LHU ambient vs submerged 1.png}
        \caption{Load-hold-unload test first cycle comparison of stress versus the mechanical part of the engineering strain at various humidities, including submerged.}
        \label{fig:Hum sub LHU 1}
    \end{figure}

    \begin{figure}[hbt!]
        \centering
        \includegraphics[width=0.78\linewidth, height=0.42\textheight]{figures/LHU ambient vs submerged 2.png}
        \caption{Load-hold-unload test first cycle comparison of the mechanical part of engineering strain and stress over time for different humidities, including submerged.}
        \label{fig:Hum sub LHU 2}
    \end{figure}

As seen in Figures \ref{fig:Hum sub LHU 1} and \ref{fig:Hum sub LHU 2}, the submerged results correlate with the previous trends observed in the humidity variance results. As the humidity increased until the sample was submerged, the stiffness of FAA-3 decreased. While the trends are as expected, the effects of submersion are significant. The Young's modulus of the material at 95\% RH was 244.86 MPa and this decreased to approximately 41.85 MPa when submerged. Only a 5\% change in RH leads to nearly a 5-fold difference in stiffness. This suggests that submerging a sample is not the same as a 100\% RH environment in terms of mechanical behavior. A possible explanation for this is Schroeder's paradox, that polymers have different maximum water uptake in the liquid and saturated vapor phases \cite{CHEN2023113050}, and this difference in water uptake would affect how the water molecules change the polymer bonds, which would, in turn, change the mechanical behavior.

The unload assesses any permanent (plastic) deformation in the polymer membrane. When the loaded sample was unloaded to a force near zero, it was found that plastic deformation increased with increasing temperature as expected since the slipping of molecules is easier at higher temperatures, but the influence of temperature on the plastic deformation was small. Figure \ref{fig:Temp LHU 1 eng} and Figure \ref{fig:Temp LHU 2 eng} both show significant plastic deformation but the plastic deformation does not differ much between the varying temperatures. This may be because the range of temperatures is relatively small or because all samples were submerged so they all behaved similarly. Either way, this reinforces that humidity plays a larger role on the mechanical behavior of FAA-3 than the temperature for MS DAC applications.

\subsection{Cyclic Loading Test}
\label{sec:Cyclic Loading Results}
Figure \ref{fig:Cyclic Loading Test 1 eng} shows the results from the cyclic loading tests, where the sample was loaded to 8\% engineering strain at an engineering strain rate of 0.0001s$^{-1}$ and then unloaded to a force near zero, for a total of 3 cycles. The stress and strain experienced by the sample over time are shown in Figure \ref{fig:Cyclic Loading Test 2 eng}.

    \begin{figure}[hbt!]
        \centering
        \includegraphics[width=0.8\linewidth, height=0.42\textheight]{figures/Cyclic Loading Test 1 eng.png}
        \caption{Cyclic loading results at \SI{27}{\celsius}, 38-41\% RH, and a strain rate of 0.0001s$^{-1}$.}
        \label{fig:Cyclic Loading Test 1 eng}
    \end{figure}
    
    \begin{figure}[hbt!]
        \centering
        \includegraphics[width=0.72\linewidth, height=0.4\textheight]{figures/Cyclic Loading Test 2 eng.png}
        \caption{Cyclic loading stress and engineering strain versus time.}
        \label{fig:Cyclic Loading Test 2 eng}
    \end{figure}

As seen in the loading of the first cycle of Figure \ref{fig:Cyclic Loading Test 2 eng}, the stress increases with strain, but while the strain is increased at a constant rate, the stress is not linear near the end of the loading because of viscous and/or plasticity effects. Stress relaxation may be prevalent from the slow strain rate, causing the stress to both increase due to an applied force and decrease due to stress relaxation, and therefore the stress begins to level out. When unloading the sample to a stress of approximately zero, the stress and strain are linear as typical of elastic unload. Although the stress reaches nearly 0 MPa, the strain does not return to 0 due to plastic deformation. The developed model should be able to simulate this viscoplastic behavior, and these cyclic loading results will be used to verify the accuracy of the model.

A comparison of the first and second trials reveals differences in material behavior, which can be attributed to variations in humidity and temperature conditions. The first trial was conducted at a lower humidity and higher temperature compared to the second. This difference was evident in the resulting curves, which showed the material in the first trial to be stiffer, emphasizing the significant influence of humidity on the mechanical properties of FAA-3. Additionally, there were slight variations in plastic deformation between the two trials. The first trial exhibited more plastic deformation than the second, suggesting that temperature has a more pronounced effect on plastic deformation than humidity. Higher humidity tends to increase plastic deformation, while lower temperatures reduce it. Since the second trial, conducted at a lower temperature, exhibited less plastic deformation despite higher humidity, it can be inferred that temperature exerts a stronger influence on the plastic deformation of the material.

\section{Conclusion}
The behavior of FAA-3 was explored via experiments to quantify the tensile, cyclic, and time-dependent mechanical response of FAA-3 under hydration and temperature effects. The experiments performed were DMA, hygroscopic swell, thermal expansion, ultimate tensile, load-hold-unload, and cyclic loading tests. The DMA test examined how a material responds to changes in temperature and strain to provide insight into the viscous behavior as well as the location of the glass transition temperature. The results showed non-negligible viscous effects as the loss modulus was approximately 10$^8$ MPa throughout the test. The glass transition temperature does not occur within the range of \SI{-150}{\celsius} to \SI{200}{\celsius} but may occur around \SIrange{200}{250}{\celsius}, so glass transition is not expected for FAA-3 used in direct air capture. The hygroscopic swell results demonstrated that the hygroscopic swelling strain in the in-plane and thickness directions were similar and displayed an approximately linear trend with change in water content. The swell coefficient ($\bm{\beta}$) was found to be about 1.02-5 m$^3$/mol in the in-plane direction and  9.24x10$^{-6}$ m$^3$/mol in the thickness direction. The thermal expansion tests showed a quadratic relationship between thermal strain and change in temperature with a $\alpha_1$ of 1.31x10$^{-4}$/\SI{}{\celsius}$^2$ and $\alpha_2$ of 3.26x10$^{-3}$/\SI{}{\celsius}. The ultimate tensile test provided an initial understanding of the material behavior and properties. The elongation at break was around 13\% mechanical strain for a dry sample and did not change much when exposed to moisture. The ultimate tensile strength of FAA-3 is approximately 50 MPa in a dry state and that value decreases with moisture content. A small decrease in strength with an increase in the rate at which the sample is loaded was also observed, but the influence of this is small for the range of rates used in this work. The load-hold-unload test was conducted with varying humidities and temperatures to obtain a detailed understanding of the mechanical behavior of the material. Through this test, it was found that the load needed to pull FAA-3 to a certain strain decreases as the humidity or temperature increases, the amount of stress relaxation that occurs increases with strain but decreases with increasing humidity or temperature, and the plastic deformation increases with increasing humidity or temperature. It was also found that polymers may have different maximum water uptake in the liquid and saturated vapor phases, implied by how a 5\% change in RH led to nearly a 5-fold difference in stiffness. The significance of this finding demonstrates how water uptake affects how the water molecules change the polymer bonds, which in turn changes the mechanical behavior. The cyclic loading test was performed to provide results that can be utilized as a comparison when a model for FAA-3 is developed. 
 
Building upon the mechanical behavior of FAA-3 observed in these tests, a model can be developed to characterize its viscoplastic, stress-strain response under uniaxial tensile and cyclic loading conditions. This model will incorporate the rate, hydration, and temperature effects to obtain a comprehensive representation of the material's performance. Based on the findings of this work, and the presumed loading of FAA-3 during MS DAC, it will be critical that this model captures how humidity affects the mechanical behavior, particularly the viscoelastic response, and less emphasis may be placed on the role of temperature on the material properties. However, the temperature dependence for Young's modulus, and some plasticity parameters may be important. Once established, the model can be integrated with chemical transport to effectively predict the mechanical behavior of FAA-3 during the carbon capture process. This coupled approach ensures a more accurate simulation of the material's response within the moisture-swing system, enhancing its practical application in removing carbon dioxide from the atmosphere.
